CausalEC: A Causally Consistent Data Storage Algorithm based on Cross-Object Erasure Coding

Current causally consistent data storage algorithms use partial or full replication to ensure data access to clients over a distributed setting. We develop, for the first time, an erasure coding-based algorithm called CausalEC that ensures causal consistency for a collection of read-write objects stored in a distributed set of nodes over an asynchronous message-passing system. CausalEC can use an arbitrary linear erasure code for data storage and ensures liveness, fault-tolerance, and storage properties prescribed by the erasure code. CausalEC retains a key benefit of previous replication-based algorithms - every write operation is "local", that is, a server performs only local actions before returning to a client that issued a write operation. For servers that store certain objects in an uncoded manner, read operations to those objects also return locally. In general, a read operation to an object can be returned by a server on contacting a small subset of other servers so long as the underlying erasure code allows for the object to be decoded from that subset. Notably, unlike previous consistent erasure coding-based algorithms, CausalEC is compatible with cross-object erasure coding, where nodes encode values across multiple objects. CausalEC navigates the technical challenges of cross-object erasure coding, in particular, pertaining to re-encoding when writes update the values and ensuring that concurrent reads are served in a non-blocking manner during the transition to storing codeword symbols corresponding to the updated values.

==> eventualEC.tex <==

\section{$EventualEC$: An eventually consistent data storage protocol that uses erasure coding}
\label{app:eventual}

In this section, we present $EventualEC$, an eventually consistent data storage protocol that uses erasure coding. $EventualEC$ has the same state variables as $CausalEC$ in Fig. \ref{alg:state}, and the client protocol is also identical to $CausaLEC$. We present the server protocol in Algorithms \ref{alg:inputactions_clients_eventual}, \ref{alg:input_actions_eventual}, and \ref{alg:internal_actions_eventual}.

$EventualEC$ satsfies all the liveness properties of $CausalEC.$ In particular, the reader can verify that it satisfies all the properties in Sections \ref{sec:liveness}, \ref{sec:storagecost}, and Apppendices \ref{app:liveness}, \ref{app:storage}. 



\begin{figure}[ht] 
\begin{algorithm}[H]
\caption{Transitions for Messages from Clients} 
\label{alg:inputactions_clients_eventual}

\footnotesize
 \underline{On  {$receive\langle\texttt{write}, opid, X,v\rangle$}  from client $id$}:

$vc[s]\leftarrow vc[s]+1$
\label{line:vcincrement_eventual}

$t\leftarrow (vc,id)$

$L[X] \leftarrow L[X] \cup \{(t,v)\}$
\label{line:writeaddtolist_eventual}

$send\langle\texttt{write-return-ack}, opid\rangle$ to client $id$
\label{line:writeresponse_eventual}

$send\langle\texttt{app},X,v,t\rangle$ to all other nodes, $j\neq i$ 
\label{line:writesendapply_eventual}


for every $opid$ such that there exists $clientid \neq \texttt{localhost}, \bar{v},tvec$ such that $(clientid, opid, X, tvec, \bar{v})\in ReadL$: 


\hspace{1cm}$send\langle \texttt{read-return}, opid,v \rangle$ to client $clientid$
\label{line:sendtoread1_eventual}

\hspace{1cm}$ReadL\leftarrow ReadL - \{(clientid, opid, X, tvec, \bar{v})\}$
\label{line:read-remove1_eventual}


\underline{On $receive\langle\texttt{read},opid, X\rangle$ from client $clientid$}:

if $L[X] \neq \{\}$ \st{and $L[X].Highesttagged.tag \geq M.tagvec[X]$}: \label{line:readimmediatereturncheck1_eventual}

\hspace{1cm}$send\langle \texttt{read-return}, opid, L[X].HighestTagged.val \rangle$ to client $clientid$    \hspace{10pt} \# return locally
\label{line:readimmediatereturn_eventual}

else if  $\{s\} \in \mathcal{R}_{ObjectIndex{X}}$ \label{line:readreturnimmediatecheck2_eventual}

\hspace{1.5cm}$v\leftarrow \Psi_{\{s\}}^{ObjectIndex[X]}( M.val)$

\hspace{1.5cm} send $\langle \texttt{read-return}, opid, v \rangle$ to client $clientid$ 

\label{line:send-to-read1_eventual}
 
else:  \hspace{10pt} \# contact other nodes

\hspace{1cm}$ReadL \leftarrow ReadL\cup (clientid, opid, X, M.tagvec ,w_1, w_2, \ldots, w_N)$, where $w_{i} = \begin{cases} M.val & \textrm{if }i = s\\ \bot & \textrm{otherwise} \end{cases}$ 
\label{line:addtoreadl_eventual}

\hspace{1cm}send$\langle\texttt{val\_inq},X, M.tagvec\rangle$ to every node $j$ where $j\neq i$
\label{line:valinq_send_eventual}
\end{algorithm}

\caption{Protocol of $EventualEC$: Transitions for input actions corresponding to messages from clients at node $s$}
\end{figure}





\begin{figure}[htp!] 
\begin{algorithm}[H]
\footnotesize

\underline{On $receive\langle\texttt{del},X, t\rangle$ from node $j$}:
 
 $DelL[X] \leftarrow DelL[X] \cup \{(t,j)\}$ 
\label{line:delmessage_eventual}


\underline{On $receive\langle\texttt{val\_inq},clientid, opid,\bar{X}, wantedtagvec\rangle)$ from node $j$}:
 
if \st{there exists $v$ such that $(v,wantedtagvec[\overline{X}]) \in L[\bar{X}]$} $clientid\neq\texttt{localhost}$ and $L[\overline{X}] \neq \{\}$:

\hspace{0.5cm}$send\langle\texttt{val\_resp}$\st{$clientid, opid$}$, \overline{X},v,\cancel{wantedtagvec}\rangle$ to node $j$

else

\hspace{0.5cm} $ResponsetoValInq \leftarrow M$
\label{line:Responsetovalinqinit_eventual}


\hspace{0.5 cm} For all $X \in \mathcal{X}_{s}$


\hspace{1 cm} If $M.tagvec[X] \neq wantedtagvec[X]$: 

\hspace{1.5 cm} If there exists unique $v$ such that $(M.tagvec[X],v) \in L[X]$

\hspace{2 cm}$ResponsetoValInq.val \leftarrow \Gamma_{s,ObjectIndex(X)}
 (ResponsetoValInq.val,v,0)$

  \hspace{2 cm}$ResponsetoValInq.tagvec[X] \leftarrow \mathbf{0}$.

\hspace{2 cm}If there exists unique $w$ such that $(wantedtagvec[X],w) \in L[X]$

\hspace{2.5 cm}$ResponsetoValInq.val \leftarrow \Gamma_{s,ObjectIndex(X)} (ResponsetoValInq.val,0,w)$

  \hspace{2.5 cm}$ResponsetoValInq.tagvec[X] \leftarrow wantedtagvec[X]$.

\hspace{0.5cm} $send \langle \texttt{val\_resp\_encoded}, ResponsetoValInq,clientid,opid, X, wantedtagvec \rangle$ to node $j$.

\underline{On $receive\langle \texttt{val\_resp\_encoded},\bar{M},clientid,opid, \overline{X}, requestedtags \rangle$ from node $j$}:

For $X \in \mathcal{X}$

\hspace{0.5 cm}
$Error1[X],Error2[X] \leftarrow 0,$

$Modified\_codeword \leftarrow \bar{M}.val$

\label{line:modifiedcodeword_init_eventual}


If there exists a tuple $(clientid,opid, \overline{X},requestedtags,\overline{w}) \in ReadL$ for some $\bar{w} \in \overline{\mathcal{W}}$ \label{line:valrespencoded_readcheck_eventual}

For all $X \in \mathcal{X}_{j}$,   \label{line:valrespencoded_objectforloop_eventual}

\hspace{0.5 cm} If $requestedtags[X] \neq \overline{M}.tagvec[X]$
\label{line:metaerrorcondition_eventual}

\hspace{1.0 cm} If $\overline{M}.tagvec[X] \neq 0$ and there exists unique $(w,\overline{M}.tagvec[X])\in L[X]$
\label{line:metaerrorcondition1_eventual}

\hspace{1.5 cm}   $Modified\_codeword \leftarrow \Gamma_{s,k}
 (Modified\_codeword,w, \mathbf{0})$
 \label{line:Modifiedcodeword1_eventual}
 
 
\hspace{1.0 cm} else if $\overline{M}.tagvec[X] \neq 0$ 

\hspace{1.5 cm} $Error1[X] \leftarrow 1.$
\label{line:seterror1_eventual}

 \hspace{1.0 cm} If $Error1[X] \neq 1$ and there exists unique $v$ such that $(requestedtags[X],v)\in L[X]$
 \label{line:metaerrorcondition2_eventual}

  \hspace{1.5 cm}  $Modified\_codeword \leftarrow \Gamma_{s,k}
 (Modified\_codeword,\mathbf{0},v)$
 \label{line:Modifiedcodeword2_eventual}
 
 
 \hspace{1.0 cm} else
 
  \hspace{1.5 cm} \label{line:seterror2_eventual}$Error2[X] \leftarrow 1$
  
  
    If $\bigwedge_{X \in \mathcal{X}} Error1[X] \wedge Error2[X]=0$
  \label{line:errorcondition_eventual}  
  
\hspace{0.5cm}  $ReadL\leftarrow ReadL-\{(clientid,opid,X,requestedtags,\overline{w})\} \cup \{(clientid,opid,X,requestedtags,\overline{w})\}$, where $\overline{v} \in \overline{W}$ is generated so that $\Pi_{i}(\overline{v}) \leftarrow  \begin{cases} \Pi_i(\overline{w}) & \textrm{if  }i \neq j \\ Modified\_codeword & \textrm{if } i = j \end{cases}$ 
\label{line:valrespencoded_addtuple_eventual}

\hspace{1cm}$S\leftarrow \{i  ~|~\Pi_i(\overline{v}) \neq \bot\}$


\hspace{1cm}$\ell \leftarrow ObjectIndex[X]$


\hspace{1cm}if there exists $T \in \mathcal{R}_\ell$ such that $T \subseteq S$:
\label{line:readreturncheck_eventual}

\hspace{1.5cm}$v\leftarrow \Psi_{T}^{(\ell)} \left(\Pi_{T}(\overline{v})\right)$
\label{line:valresp_handle_decoding_eventual}

\hspace{1.5cm}if $clientid =\texttt{localhost}$:

\hspace{2cm}$L[X]\leftarrow L[X] \cup \{(v, M.tagvec[X])\}$
\label{line:readaddtolist_eventual}

\hspace{1.5cm}else:

\hspace{2cm}$send\langle \texttt{read-return}, opid, v \rangle $ to client $clientid$
\label{line:read-send-val_resp_encoded_eventual}


\hspace{1.5cm}$ReadL\leftarrow ReadL- \{(clientid,opid, {X}, requestedtags, \bar{v}): \exists \bar{v}  \textrm{ s. t. }(clientid,opid,{X}, requestedtags, \bar{v}) \in ReadL \}$
\label{line:read-remove2_eventual}

\underline{On $receive\langle \texttt{val\_resp},\text{\sout{\ensuremath{clientid, opid}}}. X,v, \cancel{requestedtags}~\rangle$ from node $j$}:

\sout{if there exists} for every $(clientid, opid)$ such that there exists $\overline{v}, tvec$ so that $(clientid, opid, X, requestedtags,\overline{v})\in ReadL$: 
\label{line:valresp_handle_condition_eventual}

{\hspace{0.5 cm}if $clientid~ \cancelto{\neq}{=} ~~~~\texttt{localhost}$ 

\hspace{1cm}$\text{\sout{\ensuremath{L[X] \leftarrow L[X] \cup  (v,tvec[X])}}}$
\label{line:valrespaddtolist_eventual}}

\hspace{0.5cm}\st{else}:
    
\hspace{1cm}$send \langle \texttt{read-return}, opid, v \rangle$ to client $clientid$ 
\label{line:valresp_handle_eventual}

\hspace{1 cm}$ReadL\leftarrow ReadL - \{ (clientid, opid, X, requestedtags, \overline{v})\}$
\label{line:read-remove3_eventual}



\underline{On receipt of \emph{app$(X,v, t)$} from node $j$}:

$InQueue \leftarrow InQueue \cup \{(j,X,v,t)\}$
\caption{Protocol of $EventualEC$: Transitions for input actions.}
\label{alg:input_actions_eventual}
\end{algorithm}


\end{figure}




\begin{figure}[htp!] 

\begin{algorithm}[H]
\footnotesize

$\texttt{Apply}\_\texttt{InQueue}$:

precondition: $InQueue \neq <>$ 

effect:

$(j,X,v,t) \leftarrow InQueue.Head$

\sout{If ${t.ts[p]\leq vc[p]}$ for all {$p\neq j$, and $t.ts[j]=vc[j]+1$:}}
\label{line:applycondition_eventual}

\hspace{1cm}$InQueue \leftarrow InQueue - \{ (j,X,v,t)\}$ 

\hspace{1cm}$vc[j]\leftarrow t.ts[j]$

\hspace{1cm} $L[X] \leftarrow L[X] \cup (t,v)$ 
\label{line:list_applyaction_eventual}


\hspace{1cm}for every $opid$ such that $(clientid,opid, X, tvec, \bar{v})\in ReadL, clientid \neq \texttt{localhost}, \text{\sout{\ensuremath{tvec[X] \leq t}}}$: 
\label{line:readreturn_apply_condition_eventual}

\hspace{1.5cm}$send \langle \texttt{read-return}, opid, v \rangle$ to client with id $clientid$
\label{line:readreturn_apply_eventual}

\hspace{1.5cm}$ReadL\leftarrow ReadL - \{ (clientid, opid, X, tvec, \bar{v})\}$
\label{line:read-remove4_eventual}


\hspace{1cm}for every $opid$ such that $(clientid,opid, X, tvec, \bar{v})\in ReadL, clientid = \texttt{localhost}, tvec[X] = t$: 
\label{line:readreturn_apply_condition2_eventual}

\hspace{1.5cm}$ReadL\leftarrow ReadL - \{ (clientid, opid, X, tvec, \bar{v})\}$
\label{line:read-remove5_eventual}



$\texttt{Encoding}$:

precondition: none

effect:

For every $X \in \mathcal{X}_{s}$ such that $L[X] \neq \{\}$ and $L[X].Highesttagged.tag > M.tagvec[X]$
\label{line:Forloopupdatetag1_eventual}

\hspace{0.5 cm} If there exists a tuple $(M.tagvec[X],val) \in L[X]$
\label{line:conditionforupdate_eventual}

\hspace{1cm} Let $v$ be a value such that $(L[X].Highesttagged, v) \in L[X].$

\hspace{1cm} $M.val \leftarrow \Gamma_{s,k}(val, v)$

\hspace{1cm} $M.tagvec[X] \leftarrow  L[X].Highesttagged.tag$
\label{line:updatetag1_eventual}

\hspace{1 cm} $R \leftarrow \{i \in \mathcal{N}: X \in \mathcal{X}_{i}\}$

\hspace{1 cm}send $\langle \texttt{del},X,L[X].Highesttagged.tag \rangle$ to all nodes in $R$
\label{line:Delete_send1+eventual}

\hspace{1 cm} $DelL[X] \leftarrow DelL[X] \cup \{L[X].Highesttagged.tag, s)\}$
\label{line:Delete_local1_eventual}


\hspace{0.5 cm} else if there exists no tuple $(\texttt{localhost}, \overline{opid}, X, tvec, \overline{w})$ in $ReadL$ with $tvec=M.tagvec$

\hspace{1 cm} Generate a unique operation identifier $opid.$
\hspace{1 cm} $ReadL \leftarrow ReadL \cup \{ (\texttt{localhost}, opid, X, M.tagvec, w_1, w_2, \ldots, w_N, ) \}$, where $w_i = \begin{cases} M.val & \textrm{if }i=s \\ \bot & \textrm{otherwise}\end{cases}$
\label{line:readlentryencoding_eventual}

\hspace{1 cm}$send \langle \texttt{val\_inq},\texttt{localhost}, opid, X, M.tagvec\rangle$ to every node $j\neq s$
\label{line:valinq_send2_eventual}

For every $X \notin \mathcal{X}_{s}$ such that $L[X] \neq \{\}$ and $L[X].Highesttagged.tag > M.tagvec[X]$
\label{line:Forloopupdatetag2_eventual}

\hspace{0.5 cm} $R \leftarrow \{i \in \mathcal{N}: X \in \mathcal{X}_{i}\}$
\label{line:Delete2_Rset_eventual}

\hspace{0.5cm}  Let $U$ be the set of all tags $t$ such that $ R \subseteq \{i \in \mathcal{N}: \exists \hat{t}, (\hat{t},i) \in DelL[X], \hat{t} \geq t\}$
\label{line:Delete2_Uset_eventual}


\hspace{0.5cm}  Let $\overline{U} = \{t \in \mathcal{T}: \exists  val, (t,val) \in L[X], t > M.tagvec[X]\}$
\label{line:Delete2_Ubarset_eventual}

 
\hspace{0.5 cm} {If $U \cap \overline{U} \neq \{\}$}
\label{line:Delete2_condition_eventual}



\hspace{1 cm} $M.tagvec[X] \leftarrow \max(U \cap \overline{U})$
\label{line:updatetag2_eventual}


\hspace{1 cm} $DelL[X] \leftarrow DelL[X] \cup \{\max(U \cap \overline{U}), s)\}$
\label{line:Delete_local2_eventual}

\hspace{1 cm} send $\langle \texttt{del},X,\max(U\cap \overline{U}) \rangle$ to all nodes
\label{line:Delete_send2_eventual}


$\texttt{Garbage}\_\texttt{Collection}$:

precondition: None

effect: 

For $X \in \mathcal{X}$

\hspace{0.5cm} {Let $S$ be the set of all tags $t$ such that $\{i: \exists \hat{t}, (\hat{t},i) \in DelL[X], \hat{t} \geq t\} = \mathcal{N}$}
\label{line:sset_eventual}



\hspace{.5 cm} $t_{max}[X] \leftarrow \max (S)$
\label{line:tmax_eventual}


\hspace{0.5 cm} Let $\overline{S}$ be the set of all tags $t$ such that $\{i: \exists (t,i) \in DelL[X]\} = \mathcal{N}$
\label{line:s1set_eventual}

\hspace{0.5cm} $T \leftarrow \{tvec[X]: \exists clientid, opid, i, \overline{w},\bar{X} \textrm{ s.t. } (clientid, opid, \bar{X}, i, tvec, \overline{w}) \in ReadL { \textrm{ and } tvec[X] < M.tagvec[X]}\}$ 
\label{line:pendingreads_eventual}

\hspace{0.5cm} If $ \big(t{max}[X]=M.tagvec[X]\big) \textrm{AND~} \big(M.tagvec[X] \in \overline{S}) \big) {\textrm{ AND~ } \big(L[X] = \{\} \textrm{ OR } L[X].Highesttagged.tag \leq M.tagvec[X]\big)}$
\label{line:GCcondition1_eventual}

\hspace{1 cm}$L[X] \leftarrow L[X] - \{(tag,v): \exists (tag,v) \in L[X] \textrm{ s.t. } tag \leq t{max}[X], tag \notin T\}$
\label{line:GC1_eventual}

\hspace{0.5cm} else if $\big(t{max}[X] < M.tagvec[X]\big) \textrm{AND~} \big(X \notin \mathcal{X}_{s}\big)$
\label{line:GCcondition3_eventual}

\hspace{1 cm}$L[X] \leftarrow L[X] - \{(tag,v): \exists (tag,v) \in L[X] \textrm{ s.t. } tag \leq t{max}[X], tag \notin T\}$
\label{line:GC3_eventual}


\hspace{0.5cm} else

\hspace{1 cm}$L[X] \leftarrow L[X] - \{(tag,v): \exists (tag,v) \in L[X] \textrm{ s.t. } tag  < t_{max}[X], tag \notin T\}$
\label{line:GC2_eventual}


\hspace{0.5 cm} $R \leftarrow \{i \in \mathcal{N}: X \in \mathcal{X}_{i}\}$
\label{line:Delete3_Rset_eventual}

\hspace{0.5 cm} { Let $U$ be the set of all tags $t$ such that $ R \subseteq \{i \in \mathcal{N}: \exists \hat{t}, (\hat{t},i) \in DelL[X], \hat{t} \geq t\}$}
\label{line:Delete3_Uset_eventual}

\hspace{0.5 cm} If $U \neq \{\}$ and $X \in \mathcal{X}_{s}$
\label{line:Delete_cond3_eventual}

\hspace{1 cm}send $\langle \texttt{del},X,max(U) \rangle$ to all nodes
\label{line:Delete_send3_eventual}

\caption{Transitions for internal actions of node $s$ in $EventualEC$}
\label{alg:internal_actions_eventual}


\end{algorithm}


\end{figure}








==> proofs_bak.tex <==

We first show that \CausalEC~ is causally consistent in Sec. \ref{sec:safety}. In sections \ref{sec:liveness}, \ref{sec:eventual}, and \ref{sec:storagecost}, we respectively show three liveness properties. In Section \ref{sec:liveness}, we show that liveness properties pertaining termination of reads. In Section \ref{sec:eventual}, we show eventual consistency, and in Sec. \ref{sec:storagecost}, we show that the in a stable state, the storage cost of the algorithm is the storage cost of the underlying erasure code.
Missing details of the proofs of the lemmas are presented in Appendices \ref{app:safety}, \ref{app:liveness}, \ref{app:eventual_proof} and \ref{app:storage}. We begin in Sec. \ref{sec:invariants} with some definitions and lemmas which are useful for all the proofs that follow. In all our proofs, we assume that the executions are well-formed. 



\textbf{Notation:} The statements and proofs will use the following notation. For state variable $S,$ its value at node $s$ at point $P$ in an execution $\beta$ is denoted by $S_s^{P}.$ For example, for an object $X$, the value of $M_s.tagvec[X]$ at point $P$ at node $s$ is denoted as $M_s.tagvec[X]^{P},$ or equivalently $M_s^{P}.tagvec[X]$



%
%
%
%
%
%
%
%
%
%\section{Safety of $CausalEC\_exp$}\label{sec:safety}
%
%
%\begin{theorem}\label{causally consistent}
%Let $\beta$ be an execution of $CausalEC\_exp$, then $\beta$ is causally consistent.
%\end{theorem}
%
%
%We first state some definitions and prove some lemmas. Later we prove Theorem \ref{causally consistent}. 
%
%\begin{definition}[Timestamp of an operation, tag of a write operation]
%If $\pi$ is an operation in an execution $\beta$ at node $s$, the \emph{timestamp} of $\pi$, denoted as $ts(\pi)$, is defined as the value of node $s$'s vector clock immediately it responds to the client that sent the operation. The tag of a write operation $w$ that is invoked at client with identifier $id$ is denoted as  $tag(w),$ and is defined to be $(ts(w),id)$.
%\end{definition}
%
%\begin{lemma}\label{unique tag}
%Every write operation has a unique timestamp. As a consequence, every write operation has a unique tag.
%\end{lemma}
% 
%\begin{proof}
%
%Every write operation is sent by a client to a unique node $s$, and every time a write message comes to node $s$, the $s$th component of node $s$'s vector clock is incremented by 1. Note that the timestamp at any given node does not decrease. Therefore, every write is associated with a unique timestamp. this means every value that introduced by a write operation is associated with a unique timestamp. Since the timestamp is one component of the tag, every write operation is associated with a unique tag as well. 
%\end{proof}
%
%
%
%
%
%
%\begin{definition}[Graph of an execution of $CausalEC\_exp$)]\label{build graph}
%We define the directed graph $G$ of execution $\beta$ with a vertex for every operation in $\beta$ as follows:
%
%(i) If $\pi_1,\pi_2$ are two operations at the same client such that $\pi_1$ returns before $\pi_2$ is invoked at the client, then there is an edge from $\pi_1$ to $\pi_2$;
%
%(ii) If $r$ is a vertex corresponding to a read operation on object $X$ with value $v\neq \bot$, then there is an edge to $r$ from the unique write $w$ that is associated with the read $r$, that is $r$ returns the value of the write $w$. 
%\end{definition}
%
%The following lemma is key to proving causal consistency.
%
%\begin{lemma}\label{lem:buffer-M-vc}
%Consider any point $P$ of an execution $\beta$ of $CausalEC\_exp$. Consider any node $s$. 
%\begin{enumerate}
%\item Consider the write operation $w$ to object $X$ such that $ts(w) = M.tag_O.ts$. Then either (i) the write operation was sent by client associated with node $s$ and the node retuned an $\ack$ to the client before $P$, or (ii) node $s$ dequeued the apply message from $w$ from its $InQueue$ as a part of an $\texttt{Apply}\_\texttt{Inqueue}$ action before $P$. 
%\item Suppose that $B[X].tag \neq \vec{0}$ for some object $X$ at point $P$. Let $w$ be the write operation such that $ts(w) = B.tag_{X}.ts.$ Then either (i) write $w$ was sent by a client associated with node $s$ and the node retuned an $\ack$ to the client before $P$, or (ii) node $s$ dequeued the apply message from $w$ from $InQueue$ as a part of an $\texttt{Apply}\_\texttt{Inqueue}$ action before $P$. 
%\item At $P$, for every item $X$, the vector clock $vc$ is at least as large as $B[X].tag.ts$
%\item At $P$, for every item $X$, the vector clock $vc$ is at least as large as $M.tag_O.ts$.
%
%\end{enumerate}
%
%Note that $3,4$ above follow from $1,2$.
%
%\end{lemma}
%
%\begin{lemma}\label{lem:tsordering}
%Let $G$ be the graph an execution $\beta$ of $CausalEC\_exp$ and let $\pi_1,\pi_2$ be two operations in $\beta$. If there is a path from operation $\pi_1$ to operation $\pi_2$ in $G$, then $ts(\pi_1)\leq ts(\pi_2)$. Furthermore $ts(\pi_1)<ts(\pi_2)$ if $\pi_2$ is a write operation.
%\end{lemma}
% 
%\begin{proof}
%
%Because of the transitive nature of $\leq,$ it suffices to show the following: for two operations $\pi_1, \pi_2$ such that there is an edge from $\pi_1$ to $\pi_2$ in $G$, we have $ts(o_1)\leq ts(o_2)$, and if $\pi_2$ is a write, $ts(\pi_1)<ts(\pi_2)$.
%
%
%If $\pi_1, \pi_2$ are two operations at the same client, then, they were issued to the same node. Since there is an edge from $\pi_1$ to $\pi_2$, $\pi_2$ was issued to a node $s$ after the node responded to $\pi_1.$ Since the timetamp at a node never decreases, we have $ts(\pi_1) \leq ts(\pi_2)$. Furthermore, if $\pi_2$ is a write, the only way there is an edge from $\pi_1$ to $\pi_2$ is if $\pi_1,\pi_2$ are issued by the same client. In this case, as a part of the local action at the node that sends a response to $\pi_2,$ the vector clock is incremented, ensuring that $ts(\pi_1) < ts(\pi_2)$.
%
%
%If $\pi_1,\pi_2$ are two operations at different clients, by construction, there is edge from $\pi_1$ to $\pi_2$ only if $\pi_2$ is a read to an object $X$, and $\pi_1$ is a write to $X$. Suppose that $\pi_2$ was issued at node $s$. Let $M, B$ denote the value and buffer variables at node $s$. Since $\pi_2$ returned the value of $\pi_1$, the action that returned the value must be one of the following actions:
%\begin{itemize}
%%\item Receipt of write message from $\pi_1$ to object $X$
%\item Receipt of read message from $\pi_2$ object $X$
%\item Receipt of $val\_resp$ or $code\_resp$  messages 
%\item $\texttt{Apply}\_\texttt{Inqueue}$ action 
%\end{itemize}
%In all cases, by examining the protocol code, we can conclude that, after the action, we have either $B[X].tag.ts = ts(\pi_1)$ or $M[X].tag.ts = ts(\pi_1)$. Lemma \ref{lem:buffer-M-vc} implies that $ts(\pi_2) \geq ts(\pi_1)$.
%\end{proof}
%
%\begin{lemma}\label{lem:DAG}
%The graph $G$ is a directed acyclic graph.
%\end{lemma}
%We prove this lemma by contradiction. Suppose there are two operations $\pi_1,\pi_2$ such that there is path from $\pi_1$ to $\pi_2$ and from $\pi_2$ to $\pi_1$.
%By Lemma \ref{lem:tsordering}, this means $ts(\pi_1)\leq ts(\pi_2)$ and $ts(\pi_2)\leq ts(\pi_1)$, implying that $ts(\pi_1)=ts(\pi_2)$, and neither $\pi_1$ or $\pi_2$ is a write operation.
%
%If $\pi_1,\pi_2$ happens at same client $c$, for client $c$ there can only be one pending operation at a time, so it cannot be the case that $\pi_1,\pi_2$ precede each other with respect to program order.
%
%If $\pi_1,\pi_2$ happens at different clients, by Definition \ref{build graph}  there must be a write operation $w$, such that there is a path from $\pi_1$ via $w$ to $\pi_2$, by Lemma \ref{lem:tsordering}, $ts(\pi_1)<ts(w)\leq ts(\pi_2)$, implying $ts(\pi_1) \neq ts(\pi_2)$, a contradiction.
%
%
%
%
%\begin{lemma}\label{decoding_is_correct}
%For any client $c$, if there is a read operation $r$ on object $X$ of client $c$ is served by its associated node $s$ with value $v$, on receipt of $code\_resp(\bar{M})$ message, then value $v$ is the value of a write operation with tag $M.tag_O$.
%\end{lemma}
% 
%\begin{proof}
%If read operation $r$ is served on receipt of $code\_resp(\bar{M})$ message, then we know node $s$ is a parity node. By examining the parity node code on receipt of $code\_resp(\bar{M})$ message, we know that read operation $r$ can be served by this message only if $M.tag_X=\bar{M}.tag_X, M.tag_Y=\bar{M}.tag_Y$. If the two coded values have the same tags, then we know the value we get by decoding is indeed the value of its corresponding tag. Now we need to show the coded value of $c,X$ in $ReadL$ also has tags $M.tag_X, M.tag_Y$. We prove this by contradiction.
%
%Assume the coded value of $c,X$ in $ReadL$ has tags other than $M.tag_X, M.tag_Y$, this means the tags in $M$ has changed after coded value of $c,X$ is put in $ReadL$, by examining the code of $CausalEC\_exp$, we know that the only action that can change the tags of $M$ is internal action $\texttt{Clear}\_\texttt{Buffer}$, and $B[X].val\neq bot$ and $B[Y].val\neq bot$, we know that $B[X].val = \bot$ when read operation $r$ is received by node $s$, so there must be a write operation from another client or a internal $\texttt{Apply}\_\texttt{InQueue}$ action that changed $B[X].val$, but these two operation will delete any tuple of object $X$ from $ReadL$, which is a contradiction that
%there is still a tuple of object $X$ in $ReadL$.
%
% 
%\end{proof}
%
%
%\begin{lemma}\label{decodable}
%Consider any execution of $CausalEC\_exp$. For any read $r$ that is associated with write $w,$ if $w=write(X,v)$, the the read returns $v$.
%\end{lemma}
%\begin{proof}
%
%At any point of an execution of our protocol, for a given object, every entry in the list $L$ or the buffer $B$ or its encoding in $M$ is associated with a unique tag, and hence a unique write operation. As a consequence, for a given object, every value response or a code response message is associated with a unique write operation. Because every read is served by a buffer, list, or entry in $M$, every read is associated with a unique write operation. We argued in Lemma \ref{decoding_is_correct} that the decoding is never erroneous, that is, the read always returns value of the write operation it is associated with.
%%Since every code-response message checks the tag of the entire group before updating the local response list, consider any execution $\beta$ of $CausalEC\_exp$. For a node $s \in \mathcal{N}_{\ell}$ for some coding group $\ell$, let $M_\ell.tags$ represent the tags 
%\end{proof}
%
%%\begin{lemma}\label{lem:bufferincreasing}
%%Consider an execution $\beta$ of $CausalEC\_exp$($\Theta$). Consider any node $s$ and any coding group $\ell$ such that $s \in \mathcal{N}_{\ell}$. Suppose that point $P_1$ we have $ts1 = B_\ell[X].tag.ts \neq \vec{0}$. 
%%\begin{enumerate}
%%\item Suppose that at point $P_2$ which comes after $P_1$ in $\beta$, we have $B_\ell[X].tag.ts = \vec{0}$ and $ts_2 =  M_\ell.tag_O.ts$. Then $ts_2 \geq ts_1$.
%%\item Suppose that at point $P_3$ which comes after $P_1$ in $\beta,$ we have $ts_3 =  B_\ell[X].tag.ts \neq \vec{0}$. Then $ts_3 \geq ts_1$.
%%\end{enumerate}
%%\end{lemma}
%
%
%
%\begin{proof}[Proof of Theorem \ref{causally consistent}]
%Consider any execution $\beta$ of $CausalEC\_exp$. Let $G$ be the graph of the execution as per Definition \ref{build graph}. In Lemma \ref{lem:DAG}, we have shown that $G$ is a directed acyclic graph. If there is a read operation $r$ on object $X$ with value $v=\bot$, by the construction of $G$, if there is a write operation $w$ on same object $X$ that there is a path from $w$ to $r$, then it must be the case that $w$ and $r$ happens at same client $c$, and $w$ precedes $r$, for node $s$ which is associated with client $c$, if node $s$ receives a write operation on object $X$ before it receives a read operation $r$ on same object $X$, $r$ never returns initial value. So this case never happens.
%  
%Now to show causal consistency, it suffices to show that there exist no operations $w, w', r$ on the same object $X$ such that $r$ returns the value of $w$, but there is path from $w$ to $r$ via $w'$ in $G$. 
%
%Lemma \ref{lem:tsordering} shows that the timestamps satisfy $ts(w) < ts(w') \leq ts(r)$. We consider two cases. 
%
%First, we consider the case where $w'$ and $r$ are issued by the same client $c$, its associated node is $s$. There is a path from $w'$ to $r$, shows that $w'$ precedes $r$ in program order, so node $s$ receives $w'$ before $r$. And $r$ returns the value of $w$, so the value of $w$ is also applied to node $s$ before $r$ completes. 
%
%The other case is that $r$ is issued by client $c$, its associated node is $s$, and $w'$ is issued by another client. $ts(w') \leq ts(r)$ shows that the vector clock of node $s$ is at least as large as the timestamp of $w'$ at the time $r$ completes. By examining the algorithm, this show either node $s$ did an internal $\texttt{Apply}\_\texttt{InQueue}$, added the value of $w'$ to node $s$, or node $s$ received a write operation $w'$ from client before $r$ terminates. So node $s$ has the value of $w'$ before $r$ terminates, and because $r$ returns value of $w$, node $s$ also has the value of $w$ before $r$ terminates. 
%
%Two cases both show that node $s$ have both values before $r$ terminates. We know that $ts(w)<ts(w')$, by observing the algorithm, node $s$ always return the value associated with biggest tag, so $r$ will gets a response with value of $w'$, which is a contradiction. So there is no such $w'$ that there is a path form $w$ via $w'$ to $r$.
%
%\end{proof}
%
%
%

\subsection{Invariants and Lemmas}
\label{sec:invariants}

We first state some definitions and prove some lemmas.

\begin{definition}[Timestamp of an operation, tag of a write operation] \label{def:ts_tag}
Let $\pi$ be an operation that terminates in an execution $\beta$ of \CausalEC~ with operation identifier $opid$ issued by a client $c \in \mathcal{C}_{s}$ with identifier $clientid$. The \emph{timestamp} of $\pi$, denoted as $ts(\pi)$, is defined as the $vc_{s}^{P}$, that is, node $s$'s vector clock at the point $P$, where:
\begin{itemize}
\item If $\pi$ is a write operation, $P$  is the first point where server $s$ sends a $\langle opid,  \texttt{write-return-ack} \rangle$ message to client $c,$
\item If $\pi$ is a read operation, $P$  is the first point where server $s$ sends a $\langle \texttt{read-return}, opid, v \rangle$ message to client $c,$ for some $v \in \mathcal{V}$. 
\end{itemize}
The tag of a write operation $w$ that is invoked at client with identifier $id$ is denoted as  $tag(w)$, and is defined to be $(ts(w),id)$.
\end{definition}

Note that timestamp is defined for all operations, whereas tag is defined only for write operations.


\begin{lemma}\label{lem:vconlyincreases}
Let $\beta$ be an execution of $CausalEC$ and let $P$ and $Q$ be two points of $\beta$ such that $P$ comes after $Q.$ Then, for any server $s$, $vc_{s}^{P} \geq vc_{s}^{Q}.$
\end{lemma}
The proof is standard and omitted.


\begin{lemma}\label{lem:uniquetag1}
Let $\pi_1$ and $\pi_2$ be two write operations in a well-formed execution $\beta$ of CausalEC. Then $tag(\pi_1) < tag(\pi_2)$ or $tag(\pi_2) < tag(\pi_1).$  
\end{lemma}

\begin{proof}
There are only two cases: (i) $\pi_1,\pi_2$ are issued from different clients, and $\pi_1, \pi_2$ are issued from the same client.

\underline{Case (i):} In this case, $tag(\pi_1).id \neq tag(\pi_2).id$
Without loss of generality, assume that $tag(\pi_1).id < tag(\pi_2).id.$ If $tag(\pi_1).vc$ and $tag(\pi_2).vc$ are comparable, then from definition, $tag(\pi_1), tag(\pi_2)$ are also comparable. If $tag(\pi).vc$ and $tag(\pi_2).vc$ are not comparable, then from the definition of the order $\prec$, we have $tag(\pi_1) < tag(\pi_2).$

\underline{Case (ii):} Because $\beta$ is informed, either $\pi_1$ is invoked after $\pi_2$ terminates, or $\pi_2$ is invoked after $\pi_1$ terminates.
Without loss of generality, assume that $\pi_1$ invoked after $\pi_2$ terminates. 
Let $s$ be the unique server such that the client belong to $\mathcal{C}_{s}.$ Let $P,Q$ respectively denote the points at which the $\langle \texttt{write},X,v\rangle$ messages from $\pi_1, \pi_2$ arrive at server $s$. Because $\pi_1$ is issued after $\pi_2$ completes, $P$ comes after $Q$ in $\beta.$ Lemma \ref{lem:vconlyincreases} implies that $vc_{s}^{P} \geq vc_{s}^{Q}.$ Furthermore, on receipt of the  $\langle \texttt{write},X,v\rangle$ message, in line \ref{line:vcincrement}, the vector clock is incremented. So we can conclude that $vc_{s}^{P} > vc_{s}^{Q}.$ Since, by definition, we have $tag(\pi_1).vc = vc_s^{P}$ and $tag(\pi_2).vc =vc_s^{Q}$, we conclude that $tag(\pi_1).vc >tag(\pi_2).vc$ which automatically implies $tag(\pi_1) > tag(\pi_2)$.
\end{proof}

The following lemma is an immediate consequence of Lemma \ref{lem:uniquetag1} and is stated without proof.

 \begin{lemma}\label{lem:uniquetag}
Every write operation has a unique timestamp. Consequently, every write operation has a unique tag.
\end{lemma}

 
 
\subsection{Safety of $CausalEC$}\label{sec:safety}

The ideas of our safety proofs are based on those in previous works in causal consistency (e.g, \cite{ahamad1995causal}). 

\begin{theorem}\label{thm:causallyconsistent}
$CausalEC$ satisfies causal consistency.
\end{theorem}

To prove Theorem \ref{thm:causallyconsistent}, we define a $\leadsto$ partial order for any execution $\beta$ that satisfies the properties of Definition \ref{def:original_causal}. 
\begin{definition}For distinct operations $\pi_1, \pi_2$ in an execution $\beta$ of \CausalEC, we define 
$ \pi_1 \leadsto \pi_2$ if:
\begin{enumerate}[(a)]
    \item $\pi_1, \pi_2$ both have timestamps in $\beta$ and $ts(\pi_1) < ts(\pi_2)$, or 
    \item $\pi_1, \pi_2$ both have timestamps with $ts(\pi_1)=ts(\pi_2),$ and $\pi_1$ is a write operation, or
    \item $\pi_1, \pi_2$ are read operations that have timestamps issued by the same client  with $ts(\pi_1)=ts(\pi_2),$, and $\pi_1 \rightarrow \pi_2,$ or
    \item $\pi_1$ has a timestamp, but $\pi_2$ does not have a timestamp in $\beta.$
\end{enumerate}
\label{def:ourcausalordering}
\end{definition}



The claim that $\beta$ is causally consistent follows from Lemmas \ref{lem:causal1}, \ref{lem:causal2} stated below. These lemmas are proved in Appendix \ref{app:safety}.

\begin{lemma}
For any execution $\beta,$ the relation $\leadsto$ is a partial order among all the operations of $\beta.$
\label{lem:causal1}
\end{lemma}

\begin{lemma}
Let $\pi$ be any read operation to object $X$ that completes in an execution $\beta.$ Then $\pi$ returns the value $v$ of a write operation $\phi$ to object $X$ in $\beta$ with $ts(\phi) \leq ts(\pi)$.
\label{lem:causal2}
\end{lemma}


\begin{proof}[Proof of Theorem \ref{thm:causallyconsistent}.]
Lemma \ref{lem:causal1} implies that $\leadsto$ is a partial order on all operations in an execution $\beta$ of \CausalEC. We show that this order satisfies properties (1) and (2) in Definition \ref{def:original_causal}. 

We first show property (1), that is: $\pi_1 \rightarrow \pi_2 \Rightarrow \pi_1 \leadsto \pi_2.$

\underline{Proof of 1. in Definition \ref{def:original_causal}}
If $\pi_1 \rightarrow \pi_2,$ then they are issued from the same client $c$. Note that $\pi_1$ terminates in $\beta$ because $\pi_2$ cannot be issued by $c$ before $\pi_1$ terminates. Therefore $\pi_1$ acquires a timestamp. If $\pi_2$ does not acquire a timestamp, then $(d)$ in Definition \ref{def:ourcausalordering} implies that $\pi_1 \leadsto \pi_2.$ We now handle the case where $\pi_2$ acquires a timestamp. 

Note that these operations send their message to the same server $s$ where $c \in \mathcal{C}_{s}.$ Since $\pi_1$ terminates before $\pi_2$ begins, the server sends a response to $\pi_1$ at a point $P$  before the point $Q$ where it responds to $\pi_2.$ Because of Lemma \ref{lem:vconlyincreases}, $vc_{s}^{Q} \geq vc_s^{P}.$ Further, since $vc_{s}^{P} = ts(\pi_1)$ and $vc_s^{P}=ts(\pi_2),$ we have $ts(\pi_1) \leq ts(\pi_2).$ If the inequality is strict, then we readily have $\pi_1 \leadsto \pi_2$ from Definition \ref{def:ourcausalordering}. 

We examine the case that $ts(\pi_1)=ts(\pi_2).$ We claim that if this is the case, then $\pi_2$ is a read. As a contradiction, if $\pi_2$ is a write, based on the server protocol in Alg. \ref{alg:inputactions_clients}, server $s$ increments the vector clock at point $Q$ before responding to $\pi_2$. Therefore, we have $vc_{s}^{Q} > vc_{s}^{P}$ which implies $ts(\pi_1) < ts(\pi_2)$ contradicting the equality of the timestamps. Therefore $\pi_2$ is a read operation, and $\pi_1$ can be a read or a write operation. In either case, (b) and (c) in Definition \ref{def:ourcausalordering}, imply that $\pi_1 \leadsto \pi_2.$


\underline{Proof of 2. in Definition \ref{def:original_causal}:}
For any read operation $\pi_2$ on object $X$ that completes with value $v$, let $S$ be the set of all write operations $w$ to object $X$ such that \begin{itemize}
    \item The value of $w$ is $v$, and 
    \item $ts(w) \leq ts(\pi_2)$
\end{itemize}

Because of Lemma \ref{lem:causal2}, we know that $S$ is non-empty. Because $\pi_2$ completes in $\beta,$ it acquires a timestamp $ts(\pi_2)$. Because every write operation acquires a unique timestamp, and every timestamp is a vector of non-negative entries, $S$ is finite. 

Let $\pi_1$ be the write with the highest timestamp in $S$. Note that $\pi_1$ is unique and well-defined because of Lemma \ref{lem:uniquetag1} combined with the fact that $S$ is non-empty and finite implies that $\pi_1$ is well-defined. We claim $\pi_1$ satisfies the necessary attributes listed in Definition \ref{def:original_causal}. 

Because $\pi_1$ is in $S$, it $\pi_1$ satisfies properties $2(a),2(b),2(c)$ in Definition \ref{def:original_causal}. We need to show that $\pi_1$ satisfies property $2(d).$ Suppose there exists write $\pi_3$ with $\pi_1 \leadsto \pi_3 \leadsto \pi_2.$ Because Lemma \ref{lem:uniquetag1} implies that $ts(\pi_3) \neq ts(\pi_1)$, Definition $\ref{def:ourcausalordering}$ implies that $ts(\pi_1) < ts(\pi_3) \leq ts(\pi_2)$. Because $\pi_1$ is the write operation with the largest timestamp among the write operations in $S$, and because $ts(\pi_3) > ts(\pi_1)$. we infer that $\pi_3$ does not belong to $S$. Because $\pi_3$ does not belong to $S$, we conclude that $\pi_3$ either does not have value $v$ or is not performed on object $X$.
\end{proof}





\subsection{Liveness: Termination of operations}
\label{sec:liveness}
\begin{theorem}\label{lem:write_terminates}
Let $\beta$ be a fair execution of \CausalEC. Suppose $s$ is a non-halting node. Every write operation $\pi$ issued by a non-halting client  $c \in \mathcal{C}_s$ eventually terminates.
\end{theorem}

\begin{proof}
The client $c \in \mathcal{C}_{s}$ sends a $\langle \texttt{write},X,v\rangle $ message to node $s$.  On receipt of this $\texttt{write},X,v$ from client $c$, node $s$ sends $ack$ back to client $c$ during this input action transition (Line \ref{line:writeresponse} in Algorithm \ref{alg:inputactions_clients}). Since node $s$ is a non-halting node, based on its protocol, the write operation eventually gets a corresponding $ack$ from node $s$. So every write operation terminates.
\end{proof}

We next describe liveness properties pertaining to termination of read operations. The liveness property, stated in Theorem \ref{lem:read_terminates_f=0} relies crucially on Lemmas \ref{lem:read-liveness} \ref{lem:error1}, \ref{lem:error2} and \ref{lem:livenessvalresp} which are stated below. Lemmas \ref{lem:error1}, \ref{lem:error2}, which are key elements of our proof, are proved in Appendix \ref{app:liveness}. 
    

 
\begin{lemma}
Let $\beta$ be an execution of \CausalEC~ and $s$ be a server. Consider any point $P$ such that there exists a tuple $(clientid,opid, X, tvec,\bar{v})$ for $id \in \mathcal{C}$ in $ReadL_s,$ where $opid$ is the identifier of read operation  $\pi$. Let $Q$ be a point after $P$ in $\beta$ such that a tuple $(clientid, opid, X, tagvec,\bar{w})$ does not exist in $ReadL_{s}$. Then server $s$ responds to read operation $\pi$ in $\beta$ with a $\texttt{read-return}$ message by point $Q$. 
\label{lem:read-liveness}
\end{lemma}

\begin{proof}
From the protocol, an element is removed from $ReadL_{s}$ in line \ref{line:read-remove1} in in Algorithm \ref{alg:inputactions_clients},  or lines \ref{line:read-remove2} or \ref{line:read-remove3} in Algorithm \ref{alg:input_actions}, 
or in line \ref{line:read-remove4}
 in Algorithm \ref{alg:internal_actions}. Based on the protocol, in each case, just before the removal of the $ReadL,$ a $\texttt{read-return}$ message to a read. Therefore, server $s$ responds to read operation $\pi$ in $\beta$ with a $\texttt{read-return}$ message by point $Q$.
\end{proof}



 \begin{lemma}
  At any point $L$ of an execution $\beta,$ for any server $s$ and for any object $X \in \mathcal{X}$,
$Error1^{s,L}[X] = 0$
 \label{lem:error1}
 \end{lemma}
 
 
 
  \begin{lemma}
  At any point $L$ of an execution $\beta,$ for any server $s$ and for any object $X \in \mathcal{X}$,
$Error2^{s,L}[X] = 0$
 \label{lem:error2}
 \end{lemma}
 
\begin{lemma}
Let $\beta$ be an execution of \CausalEC~ and $s$ be a server. Consider any point $P$ such that there exists a tuple $(clientid, opid, X, tags,\bar{w})$ in $ReadL_s$. Suppose that node $s$ receives $\langle val\_resp\_encoded, clientid,opid, X, tags, \overline{v}\rangle$ message from node $j$ at some point $Q$ before point $P$, we have: $$ \Pi_j(\bar{w}) \neq \bot$$. 
\label{lem:livenessvalresp}
\end{lemma}
\begin{proof}
We begin with the following claim:
\begin{claim}
If there is a point $R$ after $P$ where a tuple $(\overline{clientid},opid, \overline{X}, \overline{tags},\bar{v})$ does not exist in $ReadL_s^R$, then no tuple with the same operation id exists in $ReadL_s^{R}$ for any point after $R$ in $\beta.$
\label{claim:liveness1}
\end{claim}
\begin{proof}[Sketch:]
The claim follows from noting that the protocol adds a tuple to $ReadL_s$ at most once for a given operation. Since every operation has a unique $opid,$ once a tuple with operation identifier $opid$ is removed, no tuple with the same identifier can be added to $ReadL_s.$ 
\end{proof}
Based on the protocol, on receiving a $\langle \texttt{val\_resp\_encoded}, clientid, opid, X, tags, \overline{v}\rangle$ message,  server $s$ checks if an entry exists in $ReadL_s$ with operation identifier $opid$ in line \ref{line:valrespencoded_readcheck} in Algorithm \ref{alg:input_actions}. From the protocol, node $j$ sends $\texttt{val\_resp\_encoded}$ message in response to a $val\_inq$ message, which in turn is sent by node $s$ when an entry with operation identifier $opid$ is made in $ReadL_s.$ Therefore, an entry $(clientid, opid, X, tags,\bar{w})$ is added to $ReadL_s$ before point $Q$. Since the lemma hypothesis indicates a tuple with operation identifier $opid$ exists at $P$ which is after point $Q$, Claim \ref{claim:liveness1} implies that the tuple is in  $ReadL_s^Q$. Therefore, line \ref{line:valrespencoded_readcheck} returns true at point $Q$. Because of Lemmas \ref{lem:error1}, \ref{lem:error2}, the condition in line \ref{line:errorcondition} also returns true. Therefore, line \ref{line:valrespencoded_addtuple} is executed at $Q$. Based on this line, if $(clientid, opid, X, tags,\bar{u})$ is the tuple in $ReadL_s^Q,$ we infer that $\Pi_j(\overline{u}) \neq \bot.$

Finally, from the protocol, we note that for any entry  $(clientid, opid, X, tags,\bar{z})$ in $ReadL_s^R$ at any point $R$ after $Q$, we have  $\Pi_i(\bar{u}) \neq \bot \Rightarrow \Pi_i(\bar{z}) \neq \bot.$ This is because the protocol does not replace codeword entries by null entries for a given $opid$ entry in $ReadL.$ 
\end{proof}


\begin{theorem}\label{lem:read_terminates_f=0}
Let $\beta$ be a fair execution of \CausalEC and let $s$ be a server node. Then every read operation $\pi$ on object $X$ issued by a non-halting client $c \in \mathcal{C}_{s}$ terminates so long as there is at least one recovery set $S \in \mathcal{R}_{X}$ such the nodes in $S \cup \{s\}$ are non-halting nodes.
\end{theorem}

\begin{proof}

Let $\beta$ be a fair execution of \CausalEC~ satisfying the lemma hypotheses. Consider a read operation $\pi$ for object $X$ issued to a non-failing node $s;$ the read operation sends a $\langle \texttt{read}, opid,X\rangle$ message to the server. Based on the code in Algorithm \ref{alg:inputactions_clients}, if one of the conditions in line \ref{line:readimmediatereturncheck1} or line \ref{line:readreturnimmediatecheck2} is true, then the server responds to the client with a value and the read terminates. So, to show termination of $\pi,$ it suffices to focus on the case where the conditions in line \ref{line:readimmediatereturncheck1} and line \ref{line:readreturnimmediatecheck2} in Algorithm \ref{alg:inputactions_clients} are not true. In this case, based on line \ref{line:valinq_send}, a $\texttt{val\_inq}$ message is sent to every node. 
Based on the protocol, every non-failing node  eventually responds to a $\texttt{val\_inq}$ message via a $\texttt{val\_resp}$ or a $\texttt{val\_resp\_encoded}$ message. Specifically, in $\beta$, node $s$ receives a $\texttt{val\_resp}$ or  $\texttt{val\_resp\_encoded}$  message from every node in $S$. Let $P$ be the first point of $\beta$ such that at $P$, node $s$ has received a  $\texttt{val\_resp}$ or $\texttt{val\_resp\_encoded}$   message corresponding to $\pi$ from every node in $S.$ Note that the point $P$ itself is the point of receipt of the last such  message from a node in $S.$ We show that the node $s$ sends a value to the client in response to the read by or at point $P$. 
At point $P$, there are two cases: (i) there exists no entry in $ReadL$ corresponding to $\pi$, or (ii) there is an entry $(clientid, opid, X, tags,\bar{w})$ in $ReadL$ corresponding to $\pi$, where $opid$ is its identifier. In the former case, Lemma \ref{lem:read-liveness} implies that operation $\pi$  completes. We examine the later case here. 

By point $P$, every node in $S$ sends a $\texttt{val\_resp}$ or  $\texttt{val\_resp\_encoded}$ message. We claim that in fact, every node in $S$ sends a $\texttt{val\_resp\_encoded}$. To see this, note that if a node $n \in S$ sends a \texttt{val\_resp}, the code in line \ref{line:valresp_handle} in Algorithm \ref{alg:input_actions} responds to the read operation and removes the $(clientid, opid, X, tags,\bar{w})$  tuple from $ReadL.$ Since, for every operation, an entry is made into $ReadL$ corresponding to the operation at most once, and the removal of the tuple happens before point $P$, we conclude that the tuple does not exist in $ReadL$ at point $P$ - this contradicts our earlier hypothesis that such a tuple does exist. Therefore, we conclude that every node in $S$ sends a $\texttt{val\_resp\_encoded}$ message to node $s$ in response to $\pi.$ 

From Lemma \ref{lem:livenessvalresp}, we therefore conclude that $S \subseteq \{j: \Pi_j(\bar{w}) \neq \bot\}.$ Therefore line \ref{line:readreturncheck} returns true. From the protocol code lines \ref{line:read-send-val_resp_encoded}, we conclude that node $s$ eventually sends a response to the read operation $\pi$ and removes the tuple $(clientid, opid, X, tags,\bar{w})$  from ReadL. Therefore $\pi$ eventually completes.
\end{proof}
%
%\begin{lemma}\label{lem:read_terminates_f=1}
%Let $\beta$ be a fair execution of $CausalEC\_exp$ algorithm. Suppose that the number of failure nodes $f =1$. Then every read operation $\pi$ in $\beta$ issued to a non-failing node $s$ terminates. 
%\end{lemma}
%
%\begin{proof}
%For any read operation $\pi = r(X)$ from client $c$, suppose client $c$ is associated with node $s$.
%
%If node $s$ is a data node, $\pi$ is always responded by the value of highest tagged tuple. Same argument as in Lemma \ref{lem:read_terminates_f=0}.
%
%If node $s$ is a parity node, one of the following cases must be true:
%\begin{itemize}
%\item $B[X].val\neq \bot$;
%\item $(id,X,s,\bar{v}) \in ReadL$ when node $s$ receives a $write(X,v)$ from another client $\bar{id}$;
%\item $(id,X,s,\bar{v}) \in ReadL$ when node $s$ receives a $code\_resp$ message from another node, and $S = \{\bar{i}|(\bar{id},\bar{X}, \bar{i},\bar{v})\in ReadL, \bar{id}=id \} \in \mathcal{R}_O$;
%\item $(id,X,s,\bar{v}) \in ReadL$ when node $s$ performs a $\texttt{Apply}\_\texttt{InQueue}$ internal action, and $(j,X,v,t)$ is the head of $InQueue$, and $B[X].val \neq \bot, B[X].tag<t$ or $B[X].val = \bot, M.tag_O<t$;
%\item $(id,X,s,\bar{v}) \in ReadL$ when node $s$ receives a $val\_resp(X,v,t)$ from node $s'$. 
%\end{itemize}
%
%If the failed node is a parity node, then if the first four cases are not true, then: $val\_resp(X,v,t)$ will be received by node $s$ if read operation $\pi$ has not yet been responded. 
%
%If the failed node $s'$ is a data node, and $X \not \in \mathcal{X}_{s'}$, if the first four cases are not true then: $val\_resp(X,v,t)$ will be received by node $s$ if read operation $\pi$ has not yet been responded. 
%
%If the failed node $s'$ is a data node, and $X \in \mathcal{X}_{s'}$, then if the first two and last two cases are not true, then: $code\_resp(\bar{M})$ will be received by node $s$ from survived data node if read operation $\pi$ has not yet been responded. 
%
%All above messages will be received by node $s$ follows the same argument as in Lemma \ref{lem:read_terminates_f=0}. So every read operation $\pi$ eventually terminates.
%\end{proof}
%



%
%\begin{lemma}\label{write liveness}
%Let $\beta$ be a fair execution of $CausalEC\_exp$($\Theta$) where $\mathcal{H}_{i}=\mathcal{N}_{i}$ for all $i=1,2,\ldots,E$, and the generator matrices $G_1, G_2,\ldots, G_E$ can tolerate at least $f$ node failures. Suppose that the set of failing nodes $\mathcal{F} \subset \mathcal{N}$ of non-failed nodes in $\beta$ satisfies $|\mathcal{F}| < f$. Then every write operation $\pi$ issued to a non-failing node $s$ terminates.
%\end{lemma}
%
%\begin{proof}
%According to Fig. \ref{general input actions} : input actions for $CausalEC\_exp$($\Theta$), on receipt of $\writ(X,v)$ from client, node $s$ perform a series of internal computation actions before send $\ack$ back to client, and node does not fail until the operation $\pi$ gets response, so $\pi$ terminates.
%\end{proof}
%
%
%\begin{lemma}\label{read liveness}
%Let $\beta$ be a fair execution of $CausalEC\_exp$($\Theta$) where $\mathcal{H}_{i}=\mathcal{N}_{i}$ for all $i=1,2,\ldots,E$, and the generator matrices $G_1, G_2,\ldots, G_E$ can tolerate at least $f$ node failures. Suppose that the set of failing nodes $\mathcal{F} \subset \mathcal{N}$ of non-failed nodes in $\beta$ satisfies $|\mathcal{F}| < f$. Then every read operation $\pi$ issued to a non-failing node $s$ terminates.
%\end{lemma}
%
%\begin{proof}
%According to Fig. \ref{general input actions} : input actions for $CausalEC\_exp$($\Theta$), on receipt of $\rea(X)$ from client, one of the following conditions is true:
%\begin{itemize}
%\item $B_i[X].val\neq \bot$, node $s$ sends $B_i[X].val$ to client. $\pi$ terminates;
%
%\item $s\in \psi_o$, node $s$ sends $M_i.val$ to client. $\pi$ terminates.
%
%\item $L_i[X] \neq \emptyset$, node $s$ sends $L_i[X].HighestTagged.val$ to client. $\pi$ terminates.
%
%\item If none of above conditions are true, $L_i[X] = \emptyset$, this shows that node $s$ performed an internal $\texttt{Garbage}\_\texttt{Collection}$ action, and clear $L_i[X']$ for every object $X'\in \mathcal{G}_i$ to empty set. Then one of the following conditions is true:
%\begin{itemize}
%\item There is another client performing a $writ(X,v)$ operation at same node $s$ before $\pi$ terminates, node $s$ sends the value $v$ in that $writ(X,v)$ operation to client performing $rea(X)$,  $\pi$ terminates.
%
%\item There is one node $s'$ in $\mathcal{N}-\mathcal{F}$ in which $L_i[X]$ has at least one tuple, if the tag in this tuple is equal to the tag in $M_i$ of node $s$, then this value is sent to node $s$ to terminates $\pi$; if the tag in this tuple is smaller than the tag in $M_i$ of node $s$, this means there is an incoming $app()$ message containing the object value to node $s'$, then this value will be sent to node $s$ to terminates $\pi$; if the tag in this tuple is bigger than the tag in $M_i$ of node $s$, this shows that there is an incoming $app()$ message containing the object value to node $s$, then this value will be sent back to client to terminates $\pi$;
%
%\item If none of above conditions are true. Then every node performed an internal $\texttt{Garbage}\_\texttt{Collection}$ action, and clear $L_i[X']$ for every object $X'\in \mathcal{G}_i$ to empty set. So the $M_i$ at every node $\bar{s}\in \mathcal{N}_i$ contains the same tag for every object $\bar{X} \in \mathcal{G}_i$. This is ensured by $check\_status$ messages before clearing $L_i[X']$ for every object $X'\in \mathcal{G}_i$ to empty set. Because we are using a generator matrix that can tolerate at least $f$ node failures, then there is at least one repair group $S \in \mathcal{R}_{X}$ such that no node in $S$ fails, and every node in $S$ sends a $code_resp$ message back to the sever received $\pi$, and this node send the decoded value back to client. $\pi$ terminates.
%\end{itemize}
%\end{itemize}
%
%\end{proof}



%, we first state a Lemma:
%
%\begin{lemma}\label{comparable}
%if $v_1$ and $v_2$ are two values introduced by two write operation of a same object $X$, then the tags of these two write operations are comparable, that is $t_1<t_2$ or $t_1>t_2$,  where $t_1$ and $t_2$ are tags of the two write operations.
%\end{lemma}
% 
%\begin{proof}
%Lemma \ref{unique tag} shows that $t_1 \neq t_2$. 
%Then one of the following cases must be true:
%\begin{itemize}
%\item $t_1.ts>t_2.ts$ or $t_1.ts<t_2.ts$ then $t_1>t_2$ or $t_1<t_2$
%\item $t_1.ts \not >t_2.ts$ and $t_1.ts \not<t_2.ts$ then:
%\begin{itemize}
%\item $t_1.id > t_2.id$ or  $t_1.id < t_2.id$ then $t_1>t_2$ or $t_1<t_2$;
%\item $t_1.id = t_2.id$, then $v_1$ and $v_2$ are written by the same client, because clients only issue one write operation at a given time, and every write operation increase the vector clock,  $t_1.ts>t_2.ts$ or $t_1.ts<t_2.ts$. So this case never happens.
%\end{itemize}
%\end{itemize}
%
%\end{proof}

\subsection{Liveness: Eventual Consistency}
\label{sec:eventual}

We first state Lemmas \ref{lem:eventually_apply} and \ref{lem:returntagofread}, which are proved in Appendix \ref{app:eventual_proof}. 

\begin{lemma}\label{lem:eventually_apply}
Consider a fair execution $\beta$ of \CausalEC where every server is non-halting.
Consider an element $(s',X,v,t)$  $InQueue_{s}$ at server $s$ at point $P$ of $\beta$.
Then, eventually, there is a point $Q$ in $\beta$ such that the element $(s',X,v,t)$ is not in $Inqueue_{s}$ at any point after $Q$. Additionally, for any point $Q'$ that is equal to, or after $Q$ in $\beta$, $vc_{s}^{Q'} \geq t.ts.$

\end{lemma}


\begin{lemma}\label{lem:returntagofread}
Consider an execution $\beta$ of \CausalEC. Suppose $\pi$ is any read operation to object $X$ invoked at some point after point $P$ by a client in $\mathcal{C}_{s}$, where $s$ is any server. If $\pi$ completes in $\beta,$ then it returns the value $v$ which is the value of a write operation $\phi$ to object $X$ that satisfies both the following relations:
\begin{enumerate}[(a)]
    \item $tag(\phi) \geq M_s^{P}.tagvec[X]$
    \item If $L_s^{P}[X] \neq \{\},$ then, $tag(\phi) \geq L_s^{P}[X].Hihgesttagged.tag$
\end{enumerate}
\end{lemma}





\begin{theorem}\label{eventual consistent}
Let $\alpha$ be a finite execution of \CausalEC. Let $\beta$ be any infinite fair extension  of $\alpha$ where there are no additional write operation invocations in $\beta$. If every server is non-halting in $\beta$,  then, for any object $X$, there is a point $P$ of $\beta$ where every read issued to object $X$ after $P$ returns the same value.
\end{theorem}

\begin{proof}

For any object $X$, if there is no write operation on $X$ in $\alpha$, then every read operation in $\beta$ gets initial value $v_0$ based on the protocol; this satisfies the theorem. So we consider an object $X$ such that there is at least one write operation on $X$ in $\alpha$. Because $\alpha$ is a finite execution, it has a finite number of write operations. This fact combined with Lemma \ref{lem:uniquetag1} implies that there is a unique write $\pi_X$ whose tag is the maximum among all the writes in $\alpha$ to object $X$. We show that after a point $P$ in $\beta,$ every read to $X$ returns the value of $\pi_X$.


From the protocol, $\pi_X$ sends an $\langle \texttt{app},X,val,tag(\pi_X)\rangle$ message to every server. On receipt, this message is added to a servers $Inqueue.$
Lemma \ref{lem:eventually_apply} implies that there is a point $P$ in $\beta$ after which the tuple does not exist in any server in $\beta$. Based on line \ref{line:list_applyaction} in Algorithm \ref{alg:internal_actions}, at the point of removal of the tuple from $Inqueue_s$, for any server $s$, $(tag(\pi_X),val)$ belongs to $L_s[X].$ Lemma \ref{lem:returntagofread} implies that any read that begins after $P$ returns the value of a write to object $X$ with tag at least as large as $tag(\pi_X)$. However, in $\beta,$ there is no write with a tag larger than $tag(\pi_X)$ because $\pi_X$ is the write with the maximal tag. Therefore, we conclude that any read to object $X$ invoked after $P$ at any arbitrary client returns the same value - the value of the write $\pi_X.$ 
This completes the proof.
\end{proof}





\subsection{Liveness: Storage cost}
\label{sec:storagecost}

We now show that in stable state where there is no oncoming write operations, the storage cost of our algorithm is the storage cost of the underlying erasure code. It's sufficient to show that:



\begin{theorem}
Consider a fair execution $\beta$ of \CausalEC~ where every server is non-halting. Suppose that after a point $P$ in $\beta$, there are no write operations invoked in the execution. Then, 
\begin{enumerate}[(a)]
\item eventually, for every object $X$, for every server $s$, list $L_s[X]$ is the empty set $\{\}$.
\item eventually, $\texttt{Inqueue}_s = \{\}$ for every server $s$, 
\item if there is a point $Q$ such that there are no read operations invoked after $Q$ in $\beta$, then eventually, $ReadL_{s} = \{\}$ for every server $s$.
\end{enumerate}
\label{thm:storagecost}
\end{theorem}
The above theorem relies on the following key lemma, which states that no object version remains in the list $L[X]$ indefinitely in any execution. 

which is proved in Appendix \ref{app:storage}. 

\begin{lemma}
Consider a fair execution $\beta$ where every server is non-halting. Let $\pi$ be a write to object $X$ that completes in $\beta$ with value $v$. Then, there is a point $P$ in $\beta$ after which, for any non-halting server $s,$ there is no entry of the form $(tag(\pi),val)$ in $L_s[X]$ for any value $val.$
\label{lem:storagecostkey}
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm:storagecost}]

\underline{Proof of (a):} 
By the theorem hypothesis, there are a finite number of write operations in $\beta.$
From Lemma \ref{lem:storagecostkey}, for every object $X$, for every server $s$, for every write operation $\pi$ there is a point $P_{\pi,s,X}$ in $\beta$ such that $L_{s}[X]$ does not contain an element $(tag(\pi),val)$ for any val in $L_s[X].$ Let $P$ be the latest of the point $P_{\pi,s,X}$ over all write operations $\pi,$ servers $s$ and objects $X$; note that $P$ exists in $\beta$ because the number of write operations, servers and objects are all finite. At any point $\overline{P}$ after $P$, there is no element of the form $(tag(\pi),val)$ in $L_s^{\overline{P}}[X]$ for any object $X$  in $\beta$, for any server $s$. 
From Lemma \ref{lem:valuesarelegitimate} (proved in Appendix \ref{app:safety}), we know that an element $(t,v)$ exists in a list $L_s[X]$ for some server $s$ for some object $X$ only if $t$ is that of some write operation to object $X$, and $v$ is the value of that write operation. Therefore, 
we infer that $L_s[X]$ is empty after $P$.

\underline{Proof of (b):} 
It readily follows from Lemma \ref{lem:eventually_apply}

\underline{Proof of (c):} 
The hypothesis implies that there are a finite number of read operations in $\beta$. From lemma \ref{lem:read-liveness}, there is no entry $\langle clientd, opid, X, tags, \overline{w}\rangle$ in $ReadL_s$  with $clientid \neq \texttt{localhost}$, for any server $s$.


 An entry $\langle \texttt{clientid}, opid, X, tags, \overline{w}\rangle$  with $clientid \neq \texttt{localhost}$ is added to $ReadL_{s}$ only on receiving a $\texttt{read}$ message from a client at server $s$. Because the number of read operations is finite, and because lemma \ref{lem:read-liveness} implies that every read operation terminates. Further, from the protocol code, the sending of a $\texttt{read-return}$ message to operation $opid$ in line \ref{line:read-remove1} in Algorithm \ref{alg:inputactions_clients}  lines  \ref{line:read-remove2}, \ref{line:read-remove3} in Algorithm \ref{alg:input_actions} and line \ref{line:read-remove4} in Algorithm \ref{alg:internal_actions} are accompanied by removal of the corresponding entry with operation id $opid$ from $ReadL_s.$ 
Thus, eventually there is a point $Q$ after which $ReadL_s$ is does not contain any entry with $clientid \neq \texttt{localhost}.$


Because of $(a)$ there is eventually a point after which line \ref{line:Forloopupdatetag1} in Algorithm \ref{alg:internal_actions} is not satisfied for any object $X$ for any server $s$ as the list $L_s[X]$ is empty.
Since an entry $\langle \texttt{localhost}, opid, X, tags, \overline{w}\rangle$ is added to $ReadL_s$ on line \ref{line:readlentryencoding}, which is executed only if line \ref{line:Forloopupdatetag1} is true, there is a point after which such an entry is not added to $ReadL_s.$ Furthermore, such an entry is eventually cleared by executing line \ref{line:read-remove2} or \ref{line:read-remove3} in Algorithm 
\ref{alg:input_actions}. 

Therefore, there is a point $Q$ after which $ReadL_s$ is empty in $\beta.$


\end{proof}




